Intuitively Assessing ML Model Reliability through Example-Based Explanations and Editing Model Inputs

Interpretability methods aim to help users build trust in and understand the capabilities of machine learning models. However, existing approaches often rely on abstract, complex visualizations that poorly map to the task at hand or require non-trivial ML expertise to interpret. Here, we present two visual analytics modules that facilitate an intuitive assessment of model reliability. To help users better characterize and reason about a model's uncertainty, we visualize raw and aggregate information about a given input's nearest neighbors. Using an interactive editor, users can manipulate this input in semantically-meaningful ways, determine the effect on the output, and compare against their prior expectations. We evaluate our interface using an electrocardiogram beat classification case study. Compared to a baseline feature importance interface, we find that 14 physicians are better able to align the model's uncertainty with domain-relevant factors and build intuition about its capabilities and limitations.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> discussion-old.tex <==
\section{Discussion and Future Work}

In this paper, we present two visual analytics modules to facilitate intuitive assessment of a machine learning model's reliability. 
These modules are designed to allow users to interactively probe the model and to reason about its behavior through familiar examples grounded in their domain knowledge.
Users can explore a given input's nearest neighbors in the training data to better understand if and why the model is uncertain, and what high-level features the model is learning.  
They can further manipulate the input using domain-specific transformations to test hypotheses about the model's behavior or ensure that it is not overly sensitive to small changes.  
% Through think-aloud studies with 9 physicians/medical students, we demonstrate that our interface helped participants understand the model's reasoning and uncertainty in terms of domain-relevant concepts while building intuition around its capabilities and limitations.  The interface modules we present indicate a promising direction for future work aiming to build ML systems that are useful and trustworthy to their real-world users.

Throughout think-aloud studies with 14 medical practitioners, we found that our visual analytics modules successfully achieved our design goals by helping participants reason about and interact with the model's output in ways that aligned with their domain expertise and thinking. 
Our designs were motivated in part by prior work in cognitive psychology suggesting that people solve problems by utilizing knowledge about past cases~\cite{renkl_example-based_2009,aamodt_case-based_1994}, and that it is a particularly relevant form of reasoning in medicine~\cite{sayre2017case}. Here, we demonstrate how these ideas could translate to an ML application, and their benefits for understanding model behavior. In particular, viewing nearest neighbor examples helped participants discover higher-level morphologies that the model was learning, more so than seeing important segments highlighted on the input as in our baseline.  

We also found that our interfaces helped participants approach the model in a more critical way, investigating the nearest neighbor class distribution and waveforms to see why the model was uncertain, and connecting that uncertainty to clinical concepts.  
Prior interview studies with medical practitioners have reported that \textit{``participants implicitly and explicitly understood that no tool (or person) is perfect,''}~\cite{cai2019hello}, and \textit{``the acknowledgement of this challenge promotes trustworthiness''}~\cite{tonekaboni2019clinicians}. We build upon this idea in our work, identifying and implementing specific design goals to communicate model uncertainty/limitations, and demonstrating multiple ways that participants used the resultant interfaces to understand and build trust with the model. 

%Our results provide additional evidence that understanding the ways in which a model is uncertain or unreliable does not damage trust in the model, but is actually useful for building it.
% Importantly, developing an understanding that the model is unsure or unreliable for some cases does not damage a user's trust in the model, but is actually necessary for building it. 
%Our results support findings from prior interview studies with medical practitioners including from Cai et al.~\cite{cai2019hello}, who find \textit{``participants implicitly and explicitly understood that no tool (or person) is perfect,''} and Tonekaboni et al.~\cite{tonekaboni2019clinicians}, who describe that \textit{``the acknowledgement of this challenge promotes trustworthiness.''} 
% In other words, when users can explore and understand the model's uncertainty, it further helps align the system with domain expectations that some cases are difficult and/or ambiguous, and that no system or tool is perfect.  

The input editor further allowed participants to engage in back-and-forth questioning to formulate and test their hypotheses about the model's behavior. Several studies or frameworks of interpretability needs have described the need for users to ``sanity check'' a model's decision as a way to build trust~\cite{bhatt_explainable_2020,tonekaboni2019clinicians,hong2020human,cai2019hello,liao2020questioning}, but there have been few proposed methods or interfaces for addressing this need in practice. Here, we found that our interactive input editor, which offers semantically-meaningful and domain-specific transformations, provides an effective way for users to perform such sanity checks. Importantly, we found that participants in our study described the transformations they were applying in terms of higher-level features corresponding to their domain knowledge.  

% In particular, we posit that the interactivity of the editor\,---\,giving people the ability engage in back-and-forth probing of the model\,---\,is more effective to this end than, say, presenting a score representing the model's reliability. 

In contrast, the baseline\,---\,which implemented a commonly-used feature importance method~\cite{ribeiro_why_2016}\,---\,did not facilitate the same sorts of investigation.
We found that this interface demanded too large mental leap from participants in order to to understand how highlighted important sections of the waveform contributed to a high predicted probability.
This observation is in line with prior work studying the effect of feature-based explanations on doctors' diagnostic performance~\cite{bussone_role_2015}, in which participants expressed confusion about the clinical meaning of a predicted probability, and how to incorporate the explanation into decision-making. Our study builds on these findings by specifically comparing feature-based explanations to example-based ones, describing the ways in which the latter helped participants better grasp the model's behavior and uncertainty.

At the same time, our results also point to limitations with the current design of our visual analytics interfaces and suggest opportunities for future work. 
We found that when the nearest neighbor waveforms looked significantly different than expected, participants had difficulty reasoning about why the model thought the neighbors were similar. 
We posit that part of participants' confusion was caused by the uneven distribution of beat classes in the training data, which affects the quality of nearest neighbors.
For example, supraventricular ectopic beats comprise only 2.7\% of training examples; thus, the model was neither able to precisely distinguish this beat from others, nor were there sufficient similar examples to fill the list of neighbors. 
However, this possibility of under-representation in the training data did not occur to participants when seeing low-quality neighbors. 
Aside from collecting sufficient data to compute high quality neighbors, this suggests the need for transparent communication of the model's training data distribution and its implications. 
% the nearest neighbors for some examples are lower quality, as the training data unevenly represented different classes (see \todo{Section 3.3.1}).  
% Supraventricular ectopic beats, for instance, made up only 2.7\% of the training examples.  
% As a result, the model was not able to distinguish this beat from others to the same level of detail or accuracy.
% not able to learn in as much detail or accuracy what it is that makes these beats similar to each other and differentiates them from other classes.
% Additionally, because there are simply fewer examples from this class, it is less likely that an example will have nearest neighbors that look very similar to it. 
% This consideration of under-representation in the training data, however, did not naturally occur to participants upon seeing the lower-quality neighbors.  
% This observation has a few implications for future work.  First, it motivates additional data collection to train models and compute nearest neighbors with data that is more evenly distributed across classes and other important features.  More immediately, it suggests the need to be transparent to users about under-representation in the data, and to explain its implications on quality of nearest neighbors.  
If a user is then presented with output where the neighbors do not appear to make sense, they may be better equipped to understand why this might be the case. 
Indeed, we found that when we described this phenomena to participants after the conclusion of the study, they were able to understand why under-representation would affect the nearest neighbors\,---\,it had just not been on their radar previously. Similarly, Cai et al. \cite{cai2019hello} found the need for an \textit{``AI Primer''} for users to explain, in part, \textit{``AI-specific behavior that may be surprising.''} Our observations suggest specific use cases of and types of information to include in such a primer. 

In some cases, participants found it difficult to apply transformations using the input editor because the space of possible hypotheses was too open-ended.
Here, methods that generate counterfactual examples (i.e., similar example(s) that are classified differently)~\cite{wachter_counterfactual_2018,goyal_counterfactual_2019,mothilal2020explaining} might provide useful inspiration. 
These methods automatically generate modified inputs by finding small transformations that yield different predictions, but because they do not require any user intervention, they can return unrealistic examples that cannot be probed further. 
However, such methods could usefully bootstrap our input editor.
For example, automatically generated examples could help constrain the space of possible hypotheses to only those transformations that cause the greatest change in the model output.
Users could then bring their domain knowledge to bear on selecting semantically-meaningful examples to either visualize directly or as a starting point for further transformation. 
% To imagine ways this issue could be further explored and addressed, we find it useful to compare the capabilities of the editor to interpretability methods that generate counterfactual examples (i.e., similar example(s) that are classified differently)~\cite{wachter_counterfactual_2018,goyal_counterfactual_2019,mothilal2020explaining}. 
% In these cases, a modified version of the input is automatically generated by finding small transformations that lead to different predictions\,---\,while this doesn't require the user to generate their own hypothesis, it can also return unrealistic examples that do not permit further probing.  
% With the editor, users who are familiar with the data are instead able to modify the input in ways they believe should be meaningful given their prior knowledge of and familiarity with the domain. However, as we found, this can make the interaction \textit{too} open-ended in some cases. Here, we find a promising future direction in combining aspects of the two: for example, automatically determining types of transformations that lead to the most change in the output, and narrowing the user's space of hypotheses by communicating this on the interface akin to information scent \cite{pirolli1999information}.  

Finally, while we demonstrate our interface using an ECG case study, there is a significant opportunity for future work to investigate how these interface modules could be instantiated for other applications. Different data modalities will require different techniques to facilitate comparing examples and assessing variance\,---\,for example, while overlaying examples may be appropriate for signals and other image-based data, natural language data might require viewing examples separately and explicitly highlighting differences in wording. The right input modifications will also vary based on the application, and should emerge through working with the intended users. We imagine promising directions (e.g., building on Kim et al.~\cite{kim2018interpretability}) for allowing users to define and interact with meaningful high-level concepts in different types of data.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

